On the Robustness of Epoch-Greedy in Multi-Agent Contextual Bandit Mechanisms

Efficient learning in multi-armed bandit mechanisms such as pay-per-click (PPC) auctions typically involves three challenges: 1) inducing truthful bidding behavior (incentives), 2) using personalization in the users (context), and 3) circumventing manipulations in click patterns (corruptions). Each of these challenges has been studied orthogonally in the literature; incentives have been addressed by a line of work on truthful multi-armed bandit mechanisms, context has been extensively tackled by contextual bandit algorithms, while corruptions have been discussed via a recent line of work on bandits with adversarial corruptions. Since these challenges co-exist, it is important to understand the robustness of each of these approaches in addressing the other challenges, provide algorithms that can handle all simultaneously, and highlight inherent limitations in this combination. In this work, we show that the most prominent contextual bandit algorithm, $\epsilon$-greedy can be extended to handle the challenges introduced by strategic arms in the contextual multi-arm bandit mechanism setting. We further show that $\epsilon$-greedy is inherently robust to adversarial data corruption attacks and achieves performance that degrades linearly with the amount of corruption.

==> checklist.tex <==

\paragraph{Checklist:}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
\answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
\answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
\answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
\answerNA{}
  \item Did you mention the license of the assets?
\answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
\answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
\answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
\answerNA{}
\end{enumerate}

\end{enumerate}


==> related.tex <==
%Our work contributes to the literature of principal learning in auction design in repeated settings with strategic agents. Outside of pay-per-click auctions there are multiple auction settings where principal learning with strategic agents arises, . These works assume either the bidders discount their future utilities or assume that the same bidders only shows up for a limited number of rounds and thus have limited impact over principal learning. We don't make any such assumptions about the agents' behavior.  Finally, we note that repeated auction design with strategic agents also arises in many other works within dynamic mechanism design \cite{bergemann2006efficient, nazerzadeh2008dynamic, kakade2013optimal} for a non-exhaustive list. All the above works do not extend to the presence of adversarial corruptions and they also require the agents to know their exact values at the beginning of each round; in contrast, we allow learning to also arise at the agent level (Section~\ref{sec:agent_learning}).

%Our work also adds to the growing literature that deviates from assuming that agents have ex-ante information about their values but rather studies settings where they need to learn how to act on the fly. Online learning for an agent that does not know their value was initially studied in the context of second-price auctions \cite{weed2016online} and subsequently extended to more general settings \cite{feng2018learning}. 




